Program Verification via Predicate Constraint Satisfiability Modulo Theories

This paper presents a verification framework based on a new class of predicate Constraint Satisfaction Problems called pCSP where constraints are represented as clauses modulo first-order theories over function variables and predicate variables that may represent well-founded predicates. The verification framework generalizes an existing one based on Constrained Horn Clauses (CHCs) to arbitrary clauses, function variables, and well-foundedness constraints. While it is known that the satisfiability of CHCs and the validity of queries for Constrained Logic Programs (CLP) are inter-reducible, we show that, thanks to the added expressiveness, pCSP is expressive enough to express muCLP queries. muCLP itself is a new extension of CLP that we propose in this paper. It extends CLP with arbitrarily nested inductive and co-inductive predicates and is equi-expressive as first-order fixpoint logic. We show that muCLP can naturally encode a wide variety of verification problems including but not limited to termination/non-termination verification and even full modal mu-calculus model checking of programs written in various languages. To establish our verification framework, we present (1) a sound and complete reduction algorithm from muCLP to pCSP and (2) a constraint solving method for pCSP based on stratified CounterExample-Guided Inductive Synthesis (CEGIS) of (co-)inductive invariants, ranking functions, and Skolem functions witnessing existential quantifiers. Stratified CEGIS combines CEGIS with stratified families of templates to achieve relative completeness and faster and stable convergence of CEGIS by avoiding the overfitting problem. We have implemented the proposed framework and obtained promising results on diverse verification problems that are beyond the scope of the previous verification frameworks based on CHCs.

==> proof.tex <==
To prove Lemma~\ref{lem:elimmu}, we use the following lemmas.
\begin{lemma}
\label{lem:preserve}
Let $\mathcal{P}\defeq(X(\myseq{x}) =_\mu \phi');(X_i(\myseq{x}_i)=_\nu \phi_i)_{i=1}^m$ and $\mathcal{P}'\defeq(X(\myseq{x}) =_\nu \sigma_X(\phi'));(X_i(b_i,\myseq{x},\myseq{x}_i)=_\nu \sigma_i(\phi_i))_{i=1}^m$ where
\begin{align*}
\sigma_X &\defeq \finset{X \mapsto \lambda \myseq{y}.X(\myseq{y}) \land \wfp{X}(\myseq{x},\myseq{y})} \cup \myset{X_i \mapsto \lambda \myseq{y}.X_i(\top,\myseq{x},\myseq{y})}{i=1,\dots,m} & \\
\sigma_i &\defeq \finset{X \mapsto \lambda \myseq{y}.X(\myseq{y}) \land (b_i \imply \wfp{X}(\myseq{x},\myseq{y}))} \cup \myset{X_j \mapsto \lambda \myseq{y}.X_j(b_i,\myseq{x},\myseq{y})}{j=1,\dots,m} &
\end{align*}
Let $\mathit{BinReach}(Y)$ be the binary reachability relation that relates the arguments $\myseq{v}$ of $X$ with the actual arguments of each (possibly indirect\footnote{Here, we exclude indirect calls to $Y$ via another call to $X$.}) call to $Y$ caused by the call $X (\myseq{v})$.  We then have $\finset{\wfp{X} \mapsto \myset{(\myseq{v},\myseq{v}')}{\mathcal{P} \models X(\myseq{v}),\mathcal{P} \models X(\myseq{v}'),(\myseq{v},\myseq{v}') \in \mathit{BinReach}(X)}} \models \WF{\wfp{X}}$ and, for any set $\mathit{Init}$ of sequences of values of the same sort as the arguments of $X$ such that $\myset{\myseq{v}'}{\myseq{v} \in \mathit{Init},(\myseq{v},\myseq{v}') \in \mathit{BinReach}(X)} \subseteq \mathit{Init}$, and for any interpretation $\rho'$ such that $\myset{(\myseq{v},\myseq{v}')}{\myseq{v} \in \mathit{Init},(\myseq{v},\myseq{v}') \in \mathit{BinReach}(X)} \subseteq \rho'(\wfp{X})$:
\begin{itemize}
\item
$\denote{}{\mathcal{P}}(\rho)(X)(\myseq{v})
=
\denote{}{\mathcal{P}'}(\rho \uplus \rho')(X)(\myseq{v})$
for all $\myseq{v} \in \mathit{Init}$,
\item
$\denote{}{\mathcal{P}}(\rho)(X_i)(\myseq{v})
=
\denote{}{\mathcal{P}'}(\rho \uplus \rho')(X_i)(\bot,\myseq{v}',\myseq{v})$
for all $i \in \finset{1,\dots,m}$, $\myseq{v},\myseq{v}'$,
\item
$\denote{}{\mathcal{P}}(\rho)(X_i)(\myseq{v})
=
\denote{}{\mathcal{P}'}(\rho \uplus \rho')(X_i)(\top,\myseq{v}',\myseq{v})$
for all $i \in \finset{1,\dots,m}$, $\myseq{v},\myseq{v}'$ such that $\myseq{v}' \in \mathit{Init}$ and $(\myseq{v}',\myseq{v}) \in \mathit{BinReach}(X_i)$.
\end{itemize}
\end{lemma}
\begin{lemma}
\label{lem:wf}
Let $\mathcal{P}\defeq\mathcal{P}_0;(X(\myseq{x}) =_\mu \phi');(X_i(\myseq{x}_i)=_\nu \phi_i)_{i=1}^m$ and $\mathcal{P}'\defeq\sigma_0(\mathcal{P}_0);(X(\myseq{x}) =_\nu \sigma_X(\phi'));(X_i(b_i,\myseq{x},\myseq{x}_i)=_\nu \sigma_i(\phi_i))_{i=1}^m$ where
\begin{align*}
&\sigma_0 \defeq \myset{X_i \mapsto \lambda \myseq{y}.X_i(\bot,\myseq{v},\myseq{y})}{i=1,\dots,m} & \\
\sigma_X &\defeq \finset{X \mapsto \lambda \myseq{y}.X(\myseq{y}) \land \wfp{X}(\myseq{x},\myseq{y})} \cup \myset{X_i \mapsto \lambda \myseq{y}.X_i(\top,\myseq{x},\myseq{y})}{i=1,\dots,m} & \\
\sigma_i &\defeq \finset{X \mapsto \lambda \myseq{y}.X(\myseq{y}) \land (b_i \imply \wfp{X}(\myseq{x},\myseq{y}))} \cup \myset{X_j \mapsto \lambda \myseq{y}.X_j(b_i,\myseq{x},\myseq{y})}{j=1,\dots,m} &
\end{align*}
Suppose that there is an interpretation $\rho'$ of $\wfp{X}$ such that $\rho' \models \WF{\wfp{X}}$ and $\rho \uplus \rho' \models (\sigma_0(\phi),\mathcal{P}')$.  We then have $\myset{(\myseq{v},\myseq{v}')}{\myseq{v} \in \mathit{Reach}(X),\mathcal{P} \models X(\myseq{v}),\mathcal{P} \models X(\myseq{v}'),(\myseq{v},\myseq{v}') \in \mathit{BinReach}(X)} \subseteq \rho'(\wfp{X})$ where $\mathit{Reach}(X)$ represents the set of the actual arguments $\myseq{v}$ of each (possibly indirect\footnote{Here, we include indirect calls to $X$ via another call to $X$.}) call to $X$ caused by the query.
\end{lemma}

We now show Lemma~\ref{lem:elimmu}:
\begin{itemize}
\item \emph{``only if'' direction}: Suppose that $\rho \models (\phi,\mathcal{P};(X(\myseq{x}) =_\mu \phi');(X_i(\myseq{x}_i)=_\nu \phi_i)_{i=1}^m)$.  Let $\rho'=\finset{\wfp{X} \mapsto \myset{(\myseq{v},\myseq{v}')}{\mathcal{P} \models X(\myseq{v}),\mathcal{P} \models X(\myseq{v}'),(\myseq{v},\myseq{v}') \in \mathit{BinReach}(X)}}$.  By Lemma~\ref{lem:preserve}, it follows that $\rho' \models \WF{\wfp{X}}$ and $\rho \uplus \rho' \models (\sigma_0(\phi),\sigma_0(\mathcal{P});(X(\myseq{x}) =_\nu \sigma_X(\phi'));(X_i(b_i,\myseq{x},\myseq{x}_i)=_\nu \sigma_i(\phi_i))_{i=1}^m)$.
\item \emph{``if'' direction}: Suppose that there is an interpretation $\rho'$ of $\wfp{X}$ such that $\rho' \models \WF{\wfp{X}}$ and $\rho \uplus \rho' \models (\sigma_0(\phi),\sigma_0(\mathcal{P});(X(\myseq{x}) =_\nu \sigma_X(\phi'));(X_i(b_i,\myseq{x},\myseq{x}_i)=_\nu \sigma_i(\phi_i))_{i=1}^m)$.  By Lemma~\ref{lem:wf}, we obtain $\myset{(\myseq{v},\myseq{v}')}{\myseq{v} \in \mathit{Reach}(X),\mathcal{P} \models X(\myseq{v}),\mathcal{P} \models X(\myseq{v}'),(\myseq{v},\myseq{v}') \in \mathit{BinReach}(X)} \subseteq \rho'(\wfp{X})$.  Therefore, by Lemma~\ref{lem:preserve}, we get $\rho \models (\phi,\mathcal{P};(X(\myseq{x}) =_\mu \phi');(X_i(\myseq{x}_i)=_\nu \phi_i)_{i=1}^m)$.
\end{itemize}

